Strengthening Skeletal Action Recognizers via Leveraging Temporal Patterns

Skeleton sequences are compact and lightweight. Numerous skeleton-based action recognizers have been proposed to classify human behaviors. In this work, we aim to incorporate components that are compatible with existing models and further improve their accuracy. To this end, we design two temporal accessories: discrete cosine encoding (DCE) and chronological loss (CRL). DCE facilitates models to analyze motion patterns from the frequency domain and meanwhile alleviates the influence of signal noise. CRL guides networks to explicitly capture the sequence's chronological order. These two components consistently endow many recently-proposed action recognizers with accuracy boosts, achieving new state-of-the-art (SOTA) accuracy on two large datasets.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rebuttals/all.tex <==
\noindent
We thank all the reviewers for their valuable comments.

\noindent
\textbf{\textcolor{red}{R1}: Comparison with rank pooling in [11].} 
\highlight{CRL consistently outperforms the rank pooling, as shown in \autoref{tab:11_crl_compare}.}
%\autoref{tab:11_crl_compare} shows the comparison between rank pooling in [11] and CRL. CRL consistently outperforms rank pooling. 
We conjecture that CRL's higher accuracy is because [11] linearly transforms the feature of each frame while CRL transfers each frame’s representation using a neural network with non-linear activation. Previous work has revealed that non-linear activation enhances a model’s capability~\cite{lu2017expressive}. 

\begin{table}[h!]\small
\centering
\caption{
Comparison between the rank pooling in [11] and CRL. 
}
% \vspace{-2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c | rr  rr }
\toprule
% row 1
%\rowcolor{Gray}
&
&
\multicolumn{2}{c }{\textbf{NTU60}} 
& \multicolumn{2}{c}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
\\
% row 2
\cline{3-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} &
\multirow{-2}{*}{\textbf{Features}}  &
X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
\\
\midrule 
{[11]} & Joint & 87.6 & 93.7 & 82.1 & 84.0 \\
CRL & Joint & 88.2 & 95.2 & 82.5 & 84.3 \\
\midrule 
{[11]} & Bone & 88.6 & 94.0 & 84.4 & 85.8 \\
CRL & Bone & 89.4 & 95.3 & 84.7 & 86.6 \\
\bottomrule
\end{tabular}
}
\label{tab:11_crl_compare}
\end{table}

\noindent
\textbf{\textcolor{red}{R1}: DCE without the original sequence.}
\highlight{The results of DCE without concatenating with the original sequence are shown in \autoref{tab:no_concat}.} As stated in line\#399, concatenating frequency features with original leads to higher accuracy. %We will include the result in the final revision.

\begin{table}[h!]\small
\centering
\caption{
Results of DCE without and with the original sequence. 
}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c | rr  rr }
\toprule
% row 1
%\rowcolor{Gray}
&
&
\multicolumn{2}{c }{\textbf{NTU60}} 
& \multicolumn{2}{c}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
\\
% row 2
\cline{3-6}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} &
\multirow{-2}{*}{\textbf{Features}}  &
X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
\\
\midrule 
No-Concat & Joint & 88.0 & 94.3 & 82.5 & 83.6 \\
With-Concat & Joint & 88.5 & 95.0 & 83.1 & 85.1 \\
\midrule 
No-Concat & Bone & 89.7 & 94.8 & 85.1 & 86.1 \\
With-Concat & Bone & 90.0 & 95.1 & 85.5 & 86.6 \\
\bottomrule
\end{tabular}
}
\label{tab:no_concat}
\end{table}

% \noindent
% \textbf{\textcolor{red}{R1}: MS-G3D as the backbone}.  
% \highlight{The comparison with MS-G3D is provided in Section 4.7 (line\#802-849).} We also present the results in~\autoref{tab:sota_imp}.
%We have included the results of using MS-G3D as the backbone in Section 4.7 (line\#802-849). 
% The proposed DCE-CRL improves MS-G3D on four settings of the two datasets. Specifically, On NTU120, DCE-CRL improves the classification accuracy from 86.9\% to 87.5\% on XSub and 88.4\% to 89.1\% on XSet. On NTU60, DCE-CRL enhances the performance from 91.5\% to 91.8\% for XSub and 96.6\% to 96.8\% for XView. 

\noindent
\textbf{\textcolor{red}{R1}: [7] is published in 2015}. Changed to: \textit{Since some pioneer works by [7], [22] and many more, skeleton based action recognition has attracted increasing attention}.
% We believe [7] is important since it is an early pioneering work that applies deep learning to skeleton-based action recognition. We hence mention it early. In the related work section later, we also include works that are published more recently than 2015, such as [39] in 2018 and [2] in 2020.  
% \dw{(This question seems minor. you may shorten the answer)}

\noindent
\textbf{\textcolor{red}{R1}: [39,2,30,41,4] captures spatial interactions}. 
Changed to: \textit{Most designs focus on proposing various graph operations to capture spatial interactions. On the other hand, the temporal extractors of [2,30,41] inherit ST-GCN [39].
Relatively few works [4] propose new modules to extract temporal features.}
% they use similar convolutional procedures to capture temporal patterns. 

% We will address the comment in the final revision.
% \dw{We will address the comment in the final revision.
% We intend to emphasize that their novelties concentrate more on capturing spatial interactions by designing new graph convolution operations, meanwhile using temporal convolutions for capturing temporal patterns.} \dw{(Sorry, I don't understand the sentence, especially after meanwhile ...)}
%We did not express that these works only capture spatial interactions among joints.
%We intend to mean that their novelties concentrate more on capturing spatial interactions by designing various new graph convolution operations for skeletons, meanwhile using temporal convolutions for capturing temporal patterns. We have changed the wording to the latter expression. 

\noindent
\textbf{\textcolor{red}{R1}: Order of related work 2.2 and 2.3}.
Will exchange. 

\noindent
\textbf{\textcolor{red}{R1}: Dimension of x in line\#377}. 
We explain the idea with one-dimensional sequence in line\#377. The dimension of sequence $\mathbf{x}$ is given in line\#361 as $\R^T$, where T is the length of sequence. The dimensions of the skeleton sequence before and after transformation are explicitly given in line\#398, from $\R^{C \times T \times N \times M}$ to $\R^{(K+1)C \times T \times N \times M}$. 

\noindent
\textbf{\textcolor{red}{R1}: Studies of different $K$}.
% We will include thorough study on $K$ in the final revision. E.g., we found accuracy improves as K grows, as 
We will include a thorough study on $K$ in the supp materials. 
% One further example is given in \autoref{tab:diff_K}. 
% As shown in \autoref{tab:diff_K}, performance improves slightly as $K$ increases a bit. 
%Larger $K$ leads to higher accuracy, as shown in \autoref{tab:diff_K}, where $K = 12$. 

% \begin{table}[h!]\small
% \centering
% % \vspace{-2mm}
% \caption{
% Results of $K = 8$ and $K=12$. 
% % \dw{(Try to add the result of K=8 such that the reviewer can check the difference without reading the submitted one again. However, on the other hand, the question is more about ablation, so including these results may weaker our experiments - since the reviewer thinks we did not perform proper search for the hyperparameters.)}
% } 
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{l c | rr  rr }
% \toprule
% % row 1
% %\rowcolor{Gray}
% &
% &
% \multicolumn{2}{c }{\textbf{NTU60}} 
% & \multicolumn{2}{c}{\textbf{NTU120}}
% % & \multicolumn{2}{c }{\textbf{Kinetics}}
% \\
% % row 2
% \cline{3-6}
% %\rowcolor{Gray}
% \multirow{-2}{*}{\textbf{$K$}} &
% \multirow{-2}{*}{\textbf{Features}}  &
% X-Sub
% & X-View
% & X-Sub
% & X-Set
% % & Top-1 & Top-5 
% \\
% \midrule 
% 8 & Joint & 88.5 & 95.0 & 83.1 & 85.1 \\
% 12 & Joint & 88.7 & 95.1 & 83.4 & 85.3 \\
% \midrule 
% 8 & Bone & 90.0 & 95.1 & 85.5 & 86.6 \\
% 12 & Bone & 90.1 & 95.1 & 85.9 & 86.7 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:diff_K}
% \end{table}

\noindent
\textbf{\textcolor{red}{R1}: Number of datasets}. 
Will Change it to: \textit{two datasets, each with two distinct settings}. 

\noindent
\textbf{\textcolor{red}{R1}: BKB}. We will change it to BSL. 

\noindent
\textbf{\textcolor{ForestGreen}{R3}: DCE is hand-crafted and the measurement of chronological order is probably too coarse as shown by the experimental results}. 
The research community well received the importance of hand-crafted features, especially when they are widely compatible with existing methods, \eg, the positional encoding that improves the performance of Transformers. 
% , and it brought more attention to the importance of hand-crafted features to the research community.
%We cannot properly understand the comment since it lacks concrete details. 
DCE facilitates models in analyzing motion patterns from the frequency domain and meanwhile alleviates the influence of signal noise. CRL guides networks to explicitly capture the sequence's chronological order. The experimental results show that these two components consistently endow many recently-proposed action recognizers with accuracy boosts. 
% \dw{(I think it is not generally a good idea to say we ''We cannot properly understand the comment".)}

\noindent
\textbf{\textcolor{ForestGreen}{R3}: The results of the baseline (MS-G3D) in Table 1 is different from those reported in the original paper}. 
\highlight{The baseline model used in Table 1 is a simplified version of MS-G3D without the G3D module, as described in line\#586.} %As we have described in line 586, our baseline model is not MS-G3D, but a simplified version by omitting the G3D module.
We also included the motivation that 3D graph convolutions are time-consuming, doubling the training time if employed. 
%We also justify our choice of baseline model as we aim to augment existing models with CRL and DCE to enhance the models' capability further.

\noindent
\textbf{\textcolor{red}{R1}: MS-G3D as backbone; \textcolor{ForestGreen}{R3}: MS-G3D is not listed and compared. The improvement brought by DCE and CRL in comparison to the previously reported results is insignificant}. 
\highlight{
MS-G3D is listed and compared in Section 4.7 (line\#802-849), where it is used as the backbone. 
}
We compare the accuracy with and without applying DCE-CRL to MS-G3D. 
%We have listed and compared with MS-G3D. 
%As in the previous content of this rebuttal, we have included the results of using MS-G3D as the backbone in Section 4.7 (line\#802-849). 
Also, as Figure 1 of the paper shows, DCE and CRL are widely compatible with other existing skeleton action recognizers, consistently improving their accuracy. 
Furthermore, DCE-CRL's improvement on MS-G3D is higher than the average improvement of the latest four SOTA methods comparing to the previous SOTA approach, as shown in \autoref{tab:sota_imp}. We hence believe DCE-CRL's improvement is not insignificant. 

\begin{table}[h!]\small
\centering
\caption{
Accuracy of MS-G3D with and without DCE-CRL and the average improvement of the last four SOTA methods. 
}
\resizebox{\linewidth}{!}{
\begin{tabular}{l | rr  rr }
\toprule
% row 1
%\rowcolor{Gray}
&
\multicolumn{2}{c }{\textbf{NTU60}} 
& \multicolumn{2}{c}{\textbf{NTU120}}
% & \multicolumn{2}{c }{\textbf{Kinetics}}
\\
% row 2
\cline{2-5}
%\rowcolor{Gray}
\multirow{-2}{*}{\textbf{Methods}} &
X-Sub
& X-View
& X-Sub
& X-Set
% & Top-1 & Top-5 
\\
\midrule
MS-G3D & 91.5 & 96.6 & 86.9 & 88.4 \\
With DCE-CRL & 91.8 & 96.8 & 87.5 & 89.1 \\ \hline
Improvement (Ours) & 0.30 & 0.20 & 0.60 & 0.70 \\
Previous average & 0.25 & -0.20 & 0.60 & 0.38 \\
\bottomrule
\end{tabular}
}
\label{tab:sota_imp}
\end{table}

% \dw{(I think it's worth to highlight some important messages with a different color.)}

==> rebuttals/message.tex <==
We would like to kindly ask the Area Chair to carefully consider the rating (strong reject) written by the third reviewer. The reviewer gave three short comments. These comments contain unclear descriptions and have various factual errors.  

The first comment contains unclear descriptions. 
(a) In the first part, the reviewer seems skeptical about hand-crafted features. We believe effective hand-crafted features should not be discriminated against since the research community received their importance (such as positional encodings), especially when they are widely compatible with existing methods and can consistently improve their performance (which is our case).

(b) For the second part, the meaning of ``coarse'' in the context ``the measurement of chronological is probably too coarse'' is unclear. As discussed in line\#457-472 in the paper, the proposed chronological loss can capture three kinds of temporal orders between any two arbitrary frames. 

The reviewer says our experimental results justify the first comment. However, we believe this is not the case. The results indicate that both the proposed DCE and CRL are widely compatible with existing skeleton action recognizers and consistently improve their accuracy. 

The second and third comments contain factual errors. 

For the second comment, we have described in line\#586 that our baseline model is a simplified version of MS-G3D without a G3D module. We also include the motivation that 3D graph convolutions are time-consuming, doubling the training time if employed. 

For the third comment, we have included and compared with the results of MS-G3D in Section 4.7 (lines 802-849). We show that applying DCE and CRL to MS-G3D consistently improves MS-G3D's accuracy on all four settings of the two datasets. The improvement of each setting is higher than the average improvement of the latest four SOTA methods for the corresponding setting. We hence believe our enhancement is not insignificant. 

==> secs/relative_order.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{imgs/no_enc_epoch_29.png}  
  \caption{No encoding}
  \label{fig:no_enc_frame_diff}
\end{subfigure}
% \hspace{0.05cm}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.\linewidth]{imgs/rand_enc_epoch_29.png}
  \caption{Random encoding}
  \label{fig:rand_enc_frame_diff}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.\linewidth]{imgs/tte_epoch_29.png}
  \caption{TTE}
  \label{fig:tte_frame_diff}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.\linewidth]{imgs/chronological_order_bars.png}
  \caption{Loss values}
  \label{fig:loss_frame_diff}
\end{subfigure}
\caption{Illustration of the covered nodes (yellow nodes) of anchors (red nodes).  }
\label{fig:frame_diff}
\end{figure*}

\section{TTE's Chronological Order}
\textcolor{red}{This part has not been finished. }

% The intention of this section. 
In this section, we both theoretically and experimentally demonstrate TTE's capability in precisely preserving the action sequence's chronological order. 

% Why chronological order is important. 
Existing literature have extensively argued the chronological order's importance for action recognition. For example, it is challenging to differentiate between ``sit down'' and ``stand up'' without knowing the frames' chronological order. 

% How do current models learn chronological order.
The majority of current models for skeleton-based action recognition do not directly preserve the sequence's chronological order. Nonetheless, their internal operations may implicitly capture this information. We divide the models into two classes, depending on whether iteratively or parallelly process the sequence along the temporal direction. 

% RNN approach.
Recurrent neural networks (RNNs) are typical models that iteratively extract frame information along with the temporal evolution. Thus, they are inherently aware of the chronological relative position of each frame. Previous work also indicates that a RNN has ability in counting the number of occurrences~\cite{}. As a downside of this sequential processing manner, RNNs generally show slow training and inference speed. 

% Convolution approach.
On the other hand, many models leverage temporal convolution to parallelly capture the action's various motion patterns. Different temporal convolutional operators in the same layer simultaneously extract the local dynamical pattern of several consecutive frames. As the network layers go deeper, the captured motion features become increasingly more global and abstract. Thereby, information about the chronological order is indirectly encoded in these extracted actional features. 
Two disadvantages arise in this approach. 
Firstly, information of the relative order between two far-apart frames can only be captured after going through multiple layers' processing. This can cause distortion for the extracted information on preserving relative orders. 
Secondly, both local and global temporal pooling operations are widely applied to reduce computational costs. On the other hand, pooling also leads to uncertainty in precisely preserving relative chronological order between frames. 

% Condition of encoding that has positional information.
To circumvent the above difficulties in learning the chronological order from the input sequence, we seek an encoding that directly reflects the frames' relative ordering. 
In~\cite{}, the authors consider encoding $\mathbf{n}$ contains the sequence's order information if $\mathbf{n}_{t+1} > \mathbf{n}_{t}$ for every index $t$. 
We further relax this condition as $\mathbf{n}_{t+1} \mapsto \mathbf{n}_{t}$ for every $t$, where $\mapsto$ is either $>$ (greater than) or $<$ (less than) for all $t$. That is, the encoding values monotonically change along with the sequence indices. Hence, via comparing the encoding values, the model is able to realize the relative order of two frames. 

% TTE encodes positional information. 
We notice basis sequence of TTE $\bfb_1 = [ \cos( \frac{\pi}{T} (0 + \frac{1}{2}), ..., \cos( \frac{\pi}{T} (T - 1 + \frac{1}{2}) ) ]$ exactly satisfies the above condition since it is monotonically decreasing along with the index. Although TTE additionally accommodates the Hadamard product with $\bfx$, original action sequence $\bfx$ is also incorporated in TTE. 
Thus, basis sequence $\bfb_1$ can be simply extracted from TTE via letting $\bfb_1 \odot \bfx$ elementwisely divide $\bfx$. This implies that, in theory, TTE intrinsically encodes the sequence's chronological information. 

% Experiment validation design
We also experimentally compare the model's performance on preserving the sequence's chronological order with and without TTE. 
The model sticks to MSGCN with slight variation. 
We discard the final temporal pooling to maintain the temporal dimension. Then, we use an MLP in conjunction with a normalization to convert each temporal frame's embedding to a number between $0$ and $1$, where the normalization is to let each value subtract the minimum, divided by the difference between maximum and minimum. 
We optimize the model to output the numbers of the earlier frames to be smaller than those of the latter frames, following the constraints proposed in ~\cite{}. To this end, the loss function is formulated as: 
\begin{equation}
    \relu(f(t_i) - f(t_{i+1})), 
\end{equation}
where $f$ is the MLP that takes a frame's embedding. That is, losses occur when the values of earlier frames are larger. 

% Experimental results 
We train the above model with learning rate 0.05 for 30 epochs. Three kinds of sequences are fed into the model: (1) original sequence $\bfx$; (2) $\epsilon \odot \bfx$, where $\epsilon$ is randomly sampled from the range between 0 and 1 inclusively; (3) TTE. The second and third embeddings have the same shape to dispel the influence of additional dimensions. Value $k$ of TTE is $3$.  
% 我们需要说一下loss value是多少. 

% 这一点还是没写好, 需要写一写用的是哪个样本. 
\autoref{fig:no_enc_frame_diff},~\ref{fig:rand_enc_frame_diff} and~\ref{fig:tte_frame_diff} visually depict output value $f(t)$ of each frame $t$. Since temporal dilations are applied, the number of frames eventually reduces from $300$ to $75$. 
We observe using TTE as the input results in a steadily increasing trend along with the temporal evolution, where $f(t_{i+1})$ being no smaller than $f(t_{i})$ holds for all frame $t$. In contrast, 


% 这一点写另外两种sequence表现得不好. 




==> secs/tte/tte_chron.tex <==
\section{TTE's Chronological Order}
\textcolor{red}{This part has not been finished. }

% The intention of this section. 
In this section, we both theoretically and experimentally demonstrate TTE's capability in precisely preserving the action sequence's chronological order. 

% Why chronological order is important. 
Existing literature have extensively argued the chronological order's importance for action recognition. For example, it is challenging to differentiate between ``sit down'' and ``stand up'' without knowing the frames' chronological order. 

% How do current models learn chronological order.
The majority of current models for skeleton-based action recognition do not directly preserve the sequence's chronological order. Nonetheless, their internal operations may implicitly capture this information. We divide the models into two classes, depending on whether iteratively or parallelly process the sequence along the temporal direction. 

% RNN approach.
Recurrent neural networks (RNNs) are typical models that iteratively extract frame information along with the temporal evolution. Thus, they are inherently aware of the chronological relative position of each frame. Previous work also indicates that a RNN has ability in counting the number of occurrences~\cite{}. As a downside of this sequential processing manner, RNNs generally show slow training and inference speed. 

% Convolution approach.
On the other hand, many models leverage temporal convolution to parallelly capture the action's various motion patterns. Different temporal convolutional operators in the same layer simultaneously extract the local dynamical pattern of several consecutive frames. As the network layers go deeper, the captured motion features become increasingly more global and abstract. Thereby, information about the chronological order is indirectly encoded in these extracted actional features. 
Two disadvantages arise in this approach. 
Firstly, information of the relative order between two far-apart frames can only be captured after going through multiple layers' processing. This can cause distortion for the extracted information on preserving relative orders. 
Secondly, both local and global temporal pooling operations are widely applied to reduce computational costs. On the other hand, pooling also leads to uncertainty in precisely preserving relative chronological order between frames. 

% Condition of encoding that has positional information.
To circumvent the above difficulties in learning the chronological order from the input sequence, we seek an encoding that directly reflects the frames' relative ordering. 
In~\cite{}, the authors consider encoding $\mathbf{n}$ contains the sequence's order information if $\mathbf{n}_{t+1} > \mathbf{n}_{t}$ for every index $t$. 
We further relax this condition as $\mathbf{n}_{t+1} \mapsto \mathbf{n}_{t}$ for every $t$, where $\mapsto$ is either $>$ (greater than) or $<$ (less than) for all $t$. That is, the encoding values monotonically change along with the sequence indices. Hence, via comparing the encoding values, the model is able to realize the relative order of two frames. 

% TTE encodes positional information. 
We notice basis sequence of TTE $\bfb_1 = [ \cos( \frac{\pi}{T} (0 + \frac{1}{2}), ..., \cos( \frac{\pi}{T} (T - 1 + \frac{1}{2}) ) ]$ exactly satisfies the above condition since it is monotonically decreasing along with the index. Although TTE additionally accommodates the Hadamard product with $\bfx$, original action sequence $\bfx$ is also incorporated in TTE. 
Thus, basis sequence $\bfb_1$ can be simply extracted from TTE via letting $\bfb_1 \odot \bfx$ elementwisely divide $\bfx$. This implies that, in theory, TTE intrinsically encodes the sequence's chronological information. 

% Experiment validation design
We also experimentally compare the model's performance on preserving the sequence's chronological order with and without TTE. 
The model sticks to MSGCN with slight variation. 
We discard the final temporal pooling to maintain the temporal dimension. Then, we use an MLP in conjunction with a normalization to convert each temporal frame's embedding to a number between $0$ and $1$, where the normalization is to let each value subtract the minimum, divided by the difference between maximum and minimum. 
We optimize the model to output the numbers of the earlier frames to be smaller than those of the latter frames, following the constraints proposed in ~\cite{}. To this end, the loss function is formulated as: 
\begin{equation}
    \relu(f(t_i) - f(t_{i+1})), 
\end{equation}
where $f$ is the MLP that takes a frame's embedding. That is, losses occur when the values of earlier frames are larger. 

% Experimental results 
We train the above model with learning rate 0.05 for 30 epochs. Three kinds of sequences are fed into the model: (1) original sequence $\bfx$; (2) $\epsilon \odot \bfx$, where $\epsilon$ is randomly sampled from the range between 0 and 1 inclusively; (3) TTE. The second and third embeddings have the same shape to dispel the influence of additional dimensions. Value $k$ of TTE is $3$.  
% 我们需要说一下loss value是多少. 

% 这一点还是没写好, 需要写一写用的是哪个样本. 
\autoref{fig:no_enc_frame_diff},~\ref{fig:rand_enc_frame_diff} and~\ref{fig:tte_frame_diff} visually depict output value $f(t)$ of each frame $t$. Since temporal dilations are applied, the number of frames eventually reduces from $300$ to $75$. 
We observe using TTE as the input results in a steadily increasing trend along with the temporal evolution, where $f(t_{i+1})$ being no smaller than $f(t_{i})$ holds for all frame $t$. In contrast, 


% 这一点写另外两种sequence表现得不好. 




==> unused_files/intro_old.tex <==
\section{Introduction}
% Action Recognition is important. Skeleton-Based action recognition is important. 
% Chronological order is important to learn. 
% However, chronological order may be hard to learn. We thus need TTE. 
% Contribution. 

% Why researching skeleton-based action recognition. 
Accurately recognizing human actions is essential for a wide spectrum of applications such as human-robot interaction, sports analysis and smart health-care services. Recently, skeleton-based action recognition is attracting increasing attention. 
Technically, skeleton data are concise and lightweight, granting free of environmental noises (such as background clutter, clothing and lighting) and fast processing speed on edge devices. 
Ethically, skeletonized humans are privacy-protective and racial-unbiased, promoting fair training and predicting. 

% Chronological order is important for action recognition. 
For accurate action recognition, it is crucial to adequately capture the chronological orders of action sequences. The chronological order represents the relative temporal order between two frames, \ie{}, depicting whether a frame appears earlier or later than the other. This information offers rich clues, sometimes is even indispensable, for reliably differentiating between actions. For example, it is intuitive that distinguishing between putting on shoes and taking off shoes is almost impossible without knowing their chronological orders. 

% The chronological loss is rarely explored. 
Recent approaches of skeleton-based action recognition concentrate more on more comprehensively extracting motion patterns from the skeleton trajectories, including both spatial co-occurrences and temporal movements. In contrast, learning methods about the video-wide chronological order is relatively less explored. 

% Our proposed chronological order is non-trivial. 
In this paper, we propose the chronological loss function that can methodically guide the action recognizer to accurately capture the relative order between two frames. This is a non-trivial problem. Prior to designing the loss function, we first need to formulate proper mathematical forms that rationally reflect two frames' temporal order. We show a poor form causes illogical temporal relationships between two frames. Moreover, we also show an improper loss function causes failure in learning a sequence's chronological order. 

% The chronological order is hard to learn. 
Nonetheless, even both the chronological order's mathematical form and the loss function are properly designed, learning the video-wide temporal evolution is intrinsically challenging. People perform the same action in largely various speeds. The same action can also start at different time. The action sequences may also contain noises. 
In addition, a model usually requires multiple layers' processing to learn a frame's position within the action sequence. Information leaks along layers. Frames' positional information may not be sufficiently learned, adversely influencing capturing the chronological order. 

% We propose TTE to help learning the chronological order. 
To enable the action recognizer to accurately capture the chronological order, we propose an encoding and fuse it with the action sequence. We show that this encoding theoretically and practically facilitates the model to capture information about temporal evolution. On the other hand, the spectral frequency of the proposed encoding is controllable. Since temporal noisy pieces of an action (\eg{}, joints in wrongly estimated locations and their sudden absence at some frames) turn to contain more high-frequency signals than normal parts, we can emphasize the action sequence's low-frequency components to alleviate the noise's influence. Experimental results reveal that action sequences equipped with our proposed encoding more robustly resist noise. 

% Our contributions 
We summarize our contributions as the following:
\begin{enumerate}
    \item We propose the chronological loss that effectively guides an action recognizer to capture information about the video-wide temporal evolution. 
    \item We present the temporal trigonometric encoding. It provides additional information that is theoretically sufficient for extracting the chronological order. The proposed encoding also alleviates the adverse influence of noises. 
    \item We benchmark our proposed chronological loss and temporal trigonometric encoding on a range of latest skeleton-based action recognizers. Both our loss and the encoding further improves their accuracy. 
    \item SOTA. 
    % Maybe we also talk about SOTA. Also we
\end{enumerate}

==> unused_files/old_chron_loss.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}{.3\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{imgs/chron_loss/monotonically_increase.png}  
  \caption{Monotonous}
  \label{subfig:monotonous}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.\linewidth]{imgs/chron_loss/oscillation.png}
  \caption{Oscillating}
  \label{subfig:oscillating}
\end{subfigure}
\caption{Illustration of two sequences of chronological values that have the same loss defined in  }
\label{fig:frame_diff}
\end{figure*}

\subsection{The Chronological Loss}
% Purpose of this section. 
In this section, we propose a new loss function that explicitly enables the action recognizer to correctly capture the chronological order of an action sequence. 

% Why chronological order is important. 
The chronological order depicts a frame appears earlier or later than another frame. 
The importance of being precisely aware of an action sequence's chronological order has been extensively justified by various existing literature~\cite{}. 
As an intuitive example, it is challenging to differentiate between ``putting on shoes'' and ``taking off shoes'' without knowing the relative temporal order between two frames. 

% 
In order to implement learning the chronological order, we require seeking solutions to the two problems below: 
\begin{enumerate}
    \item What is the mathematical form that rationally expresses the relative order between two frames? 
    \item What is the loss function to correctly direct the action recognizer for accurately capturing the chronological order? 
\end{enumerate}
In the following, we separately describe the approaches to the two problems. 

% 
\subsection{The Chronological Order's Mathematical Form}
% Express the chronological order is non-trivial. 
In this part, we explain how to mathematically describe the relative order between two frames. This is a non-trivial problem. Improper forms lead to non-logical temporal relationships between two frames. For example, naively, we may directly utilize the temporal indices of the frames to indicate the relative order, since an index contains absolute positional information within a sequence. A frame's index is larger than that of another frame implies that the former frame appears earlier than the other. Nonetheless, when the action performer maintains idle for two consecutive frames, it becomes irrational to apply indices for inferring their relative temporal order. This is because the two frames intrinsically do not have a temporal order. If one swaps the two frames, the entire sequence will still remain identical.  

% The mathematical form of chronological order
In sum, to mathematically model the temporal evolution in a rational manner, we require formulating three chronological relationships: a frame appears earlier, or later than another frame, or the temporal order does not exist between them. Inspired by~\cite{2017_rank_pooling}, we assign each frame at time $t$ with a value $f_\phi(\bfh_t)$, where $\bfh_t$ is the feature of the frame at time $t$ and $\phi$ is the learnable parameter. Then, we use the relative size between $f_\phi(\bfh_t)$ and $f_\phi(\bfh_{t'})$ to indicate the temporal order between the frames at time $t$ and $t'$. That is, 
\begin{itemize}
    \item $f_\phi(\bfh_i) < f_\phi(\bfh_j)$ if and only if frame $i$ appears earlier than frame $j$.
    \item $f_\phi(\bfh_i) > f_\phi(\bfh_j)$ if and only if frame $i$ appears later than frame $j$.
    \item $f_\phi(\bfh_i) = f_\phi(\bfh_j)$ if and only if the action performer stays idle during frames $i$ and $j$.
\end{itemize}
We refer to the sequence of values $[f_\phi(\bfh_{1}), f_\phi(\bfh_{2}), ..., f_\phi(\bfh_{T})]$ as the chronological values, where $T$ is the length of sequence. 

% Chronological loss
\subsection{The Chronological Loss Function}
% Introduce the chronological loss function
We have developed a mathematical form that reflects the temporal order between two frames. Now, we aim to devise a loss function that accurately guides the chronological values to indicate the correct temporal order of an action sequence. That is, the chronological values monotonically increase along with the temporal evolution: 
\begin{align}
    \forall t: f_\phi(\bfh_{t}) \le f_\phi(\bfh_{t+1}). 
    \label{eq:chron_obj}
\end{align}

% Designing loss is non-trivial 
Creating a loss function to guide the model to satisfy the above objective is non-trivial. Poor design causes fluctuations within the sequence of chronological values. For instance, straightforwardly, to let $f_\phi(\bfh_t)$ be smaller than $f_\phi(\bfh_{t+1})$, we may directly add their difference for every two adjacent frames as the loss:
\begin{equation}
    \sum_{t=1}^{T-1} f_\phi(\bfh_t) - f_\phi(\bfh_{t+1}). 
    \label{eq:simply_add_loss}
\end{equation}
However, optimizing the above loss function unintentionally compromises the desired objective specified in~\ref{}. The problem roots in the negative loss when $f_\phi(\bfh_t) \le f_\phi(\bfh_{t+1})$. It can adversely neutralize the positive loss, resulting in undesirably overlooking the cases of $f_\phi(\bfh_t) > f_\phi(\bfh_{t+1})$ for some $t$. For example, if applying \autoref{eq:simply_add_loss} as the loss function, 
the undesired oscillating chronological values in \autoref{subfig:oscillating} has the same loss with the intended monotonically increasing chronological values in \autoref{subfig:monotonous}. 

% What should a good loss function be like
Motivated by the above failure, we notice that to create a loss function that properly guides the model for fully satisfying the condition outlined in \autoref{eq:chron_obj}, we have to ensure every local decrease of the chronological values is tackled by the loss. To this end, we optimize the loss function in \autoref{eq:simply_add_loss} by leveraging the ReLU function to set the negative loss to be zero. The loss function then becomes: 
\begin{align}
     \sum_{t=1}^{T-1} \relu \bigg( f_\phi(\bfh_t) - f_\phi(\bfh_{t+1}) \bigg). 
     \label{eq:chron_loss}
\end{align}
% where 
% \begin{align}
%      \relu(x) \begin{cases}
%       x, & \text{if}\ x \ge 0 \\
%       0, & \text{otherwise}
%     \end{cases}
% \end{align}
As a result, if an earlier frame's chronological value is unintended larger than that of the following frame, a positive loss value will emerge and will not be neutralized. This loss will encourage the model to eliminate this local decrease. 
The loss value being zero if and only if the chronological values monotonically increase along with the temporal direction. 

==> unused_files/tte_old.tex <==
\subsection{Temporal Trigonometric Encoding}
\textcolor{red}{This part has not been finished. }

The proposed chronological loss function leads the action recognizer to capture information about the temporal evolution. This information is intrinsically challenging to extract for most recently proposed action recognizers. We first argue this point in the following. Then, we propose an encoding that enriches the chronological information. Also, we show this encoding alleviates the negative influence of noises. 

\textbf{Hardships in Capturing the Chronological Order}: 
We divide the recently proposed action recognizers into two classes, depending on whether iteratively or parallelly processes the sequence along the temporal direction. We demonstrate that efficiently learning the chronological order is difficult. A trade-off exists between precision and parallelization. 

% RNN approach.
(1) Recurrent neural networks (RNNs) are typical models that iteratively extract frame information along with the temporal evolution. Previous work indicates that a RNN has ability in counting the number of occurrences~\cite{}. Thus, they are inherently aware of the chronological relative position of each frame. As a downside of this sequential processing manner, RNNs generally show slow training and inference in processing sequences. 

% Convolution approach.
(2) On the other hand, many models leverage temporal convolution to parallelly capture the action's various motion patterns. Different temporal convolutional operators in the same layer simultaneously extract the local dynamical pattern of several consecutive frames. As the network layers go deeper, the captured motion features become increasingly more global and abstract. Nonetheless, information of the relative order between two far-apart frames can only be captured after going through multiple layers' processing. This can cause distortion for the extracted information on preserving relative orders. 

\textbf{Encoding the Chronological Order}: 
% Condition of encoding that has positional information.
To circumvent the above difficulties in learning the chronological order from the input sequence, we seek an encoding that directly reflects the frames' temporal relative ordering. 

We notice that a monotonically increasing function along the temporal direction encodes the relative order between two frames. A frame's value of the function is smaller than another indicates that the former frame appears earlier than the other. 

% The action performers stay still. 



This is a non-trivial problem. Improper forms lead to illogical temporal relationships between two frames. For example, naively, we may directly utilize the temporal indices of the frames to indicate the relative order, since an index contains absolute positional information within a sequence. A frame's index is larger than that of another frame implies that the former frame appears earlier than the other. Nonetheless, when the action performer maintains idle for two consecutive frames, it becomes irrational to apply indices for inferring their relative temporal order. This is because the two frames intrinsically do not have a temporal order. If one swaps the two frames, the entire sequence will still remain identical.  

% The mathematical form of chronological order
In sum, to mathematically model the temporal evolution in a rational manner, w


In~\cite{}, the authors consider encoding $\mathbf{n}$ contains the sequence's order information if $\mathbf{n}_{t+1} > \mathbf{n}_{t}$ for every index $t$. 
We further relax this condition as $\mathbf{n}_{t+1} \mapsto \mathbf{n}_{t}$ for every $t$, where $\mapsto$ is either $>$ (greater than) or $<$ (less than) for all $t$. That is, the encoding values monotonically change along with the sequence indices. Hence, via comparing the encoding values, the model is able to realize the relative order of two frames. 

% TTE encodes positional information. 
We notice basis sequence of TTE $\bfb_1 = [ \cos( \frac{\pi}{T} (0 + \frac{1}{2}), ..., \cos( \frac{\pi}{T} (T - 1 + \frac{1}{2}) ) ]$ exactly satisfies the above condition since it is monotonically decreasing along with the index. Although TTE additionally accommodates the Hadamard product with $\bfx$, original action sequence $\bfx$ is also incorporated in TTE. 
Thus, basis sequence $\bfb_1$ can be simply extracted from TTE via letting $\bfb_1 \odot \bfx$ elementwisely divide $\bfx$. This implies that, in theory, TTE intrinsically encodes the sequence's chronological information. 




% Original part. 
In skeleton-based action recognition literature, extracting patterns from temporal sequences often relies on temporal convolution. The input features are usually joint coordinates or bones (coordinate difference between adjacent joints)~\cite{shi2019two}. As in \autoref{fig:noise_sample_front}, we often observe noise in coordinates, resulting in wobbling of nodes in the temporal dimension. Models often misinterpret this as a fast movement, negatively affecting classification accuracy. %We aim to encode the coordinates of temporal sequences as a form that is more smooth and contains less noise.
Although some actions contain fast movements, one can distinguish them from coordinate noise because 1) there is a physical limit to motion speed, and 2) noise in coordinates often exhibits oscillating patterns over spatial locations as in \autoref{fig:noise_sample_front}.

If we look closer at the oscillation of spatial locations over consecutive frames, we find that the center of oscillation tends to follow the original action's trajectory, with a small displacement over the frames. The underlying trajectory is reflected in a low-frequency movement signal. In contrast, the oscillation can be wiewed as a high-frequency signal not affecting the actor's main trajectory. We can thus reduce the noise by filtering out high-frequency signals while passing the low-frequency components. 
% we propose a new encoding that extracts low-frequency signals while ignoring high-frequency components. 
% can filter out high-frequency signals while keeping the low-frequency components.

To perform this filtering, we need to decompose the signals into representations over different frequencies. However, naively feeding the DCT-transformed representations to existing skeleton-based action recognition models performs poorly, since they were not designed for processing frequency domain signals. Furthermore, standard practice usually concatenates multiple input features to enrich the input information. Nevertheless, we cannot simply concatenate  transformed frequency domain signals  with the original time domain sequence, 
% we are concatenating a frame's features with the signals of a certain frequency, 
as the physical meaning is unclear. 

Our experimental results in x support this: x depicts the classification accuracy of a common spatial-temporal GCN on the NTU120 cross-subject setting. 
If we instead feed the model with the representations transformed by DCT-2, the accuracy drops from 81.9\% to 73.7\%.
Furthermore, given a tensor $\F \in \R^{C \times T \times N \times M}$ of an action sequence, concatenating the signals transformed by DCT-2 with the $C$ (channel-wise) and $T$ (temporal-wise) axis results in a great disparity in accuracy. 
It remains non-obvious how to combine features from the two domains. 

% To keep the low-frequency components while removing high-frequency one, we propose a new encoding scheme inspired by discrete cosine transforms (DCTs). DCT transforms an input signal in the time domain to representations in the frequency domain, which can be decomposed into low- and high-frequency components.\yl{ If we naively use these transformed inputs with the previously proposed models, they will not \st{work properly} \SA{achieve the goal} since they are not compatible with the frequency domain representations.} Furthermore, in standard practice, usually multiple input features are concatenated to enrich the input information. In such a case, it also remains non-trivial how to combine the transformed signals with the original sequence in the time domain.  \SA{Hence,} it is not very \st{sensible} \SA{practical} to concatenate the two representations mechanically.



%One of our major insights is that a set of consecutive frames having more incorrect skeletons is expected to have more high-frequency signals. Thus, we intend to propose an encoding that is primarily comprised of low-frequency signals. We propose temporal trigonometric encoding (\tmodel) inspired by discrete cosine transforms (DCTs)~\cite{} and nonrigid structure from motion~\cite{}.

%To keep the low-frequency components while removing high-frequency components, we propose a new encoding scheme (\tmodel) inspired by discrete cosine transforms (DCTs)\cite{}.

%We intend to transform an arbitrary sequence of consecutive frames to the signals that preserve its low-frequency information while filtering out its high-frequency messages. DCTs can achieve this desirability. However, the transformed signals by a DCT are not compatible with the existing models for skeleton-based action recognition since the models are not designed to process representations in the frequency domain. Furthermore, we also desire to concatenate the transformed signals by a DCT with the original sequence to ensure information losslessness. It also remains non-trivial how to combine the transformed signals by a DCT with the original sequence. Specifically, the two representations are from different domains, and thus it is not very sensible to concatenate the two representations mechanically.

Our goal is to design an encoding mechanism that satisfies two requirements: 
1) it supports disentangling high- and low-frequency components of a sequence; 2) it can be meaningfully concatenated with the original sequence.
Signal transformation approaches like DCTs are a linear combination of a collection of basis sequences. Given a sequence $\X = [x_0, \cdots, x_{T-1}]^\top \in \R^{T}$, the $k$-th basis sequence of DCT-2 is: 
% i) it contains less high-frequency information; ii) it can be concatenated with the original sequence in a meaningful fashion; iii) the concatenated form is compatible with the existing models for skeleton-based action recognition. \st{To this end, we notice} \SA{The} signal transformation approaches like DCTs can be written as a linear combination of a collection of basis sequences. For example, given a sequence $\X = [x_0, \cdots, x_{T-1}]^\top \in \R^{T}$, the $k$-th basis sequence of DCT-2 (Eq.~\ref{eq:dct_2}) can be written as: 
\begin{equation}
    \B_k = \left[ \cos \left( \frac{\pi}{T} (0 + \frac{1}{2}) k \right), \cdots, \cos \left( \frac{\pi}{T} (T-1 + \frac{1}{2}) k  \right) \right]^\top, \notag 
\end{equation}
We can use this basis sequence to express the $k$-th element of the transformed sequence of $\X$ by DCT-2 (\autoref{eq:dct_2}) as: 
\begin{equation}
    \D_k = \X^\top \B_k. 
\end{equation}
% Such basis sequences are still in the domain of the original signals and thus can be concatenated with them. 
% as well as be compatible with the existing models. 
% Furthermore, we can select a set of small values of $k$ to extract low-frequency patterns within the given sequence. Formally, we denote the collection of basis sequences as $\mathbf{B} = [\B_0, \cdots, \B_{K-1}] \in \R^{K \times T}$, where $K$ is a hyperparameter controlling the complexity of $\B$. A larger $k$ corresponds to a higher frequency. Thus, selecting $K$ close to $T$ leads to $\X^\top \B$ preserving more high-frequency information of $\X$.

Motivated by this, we propose the following temporal trigonometric encodings (\tmodel) as additional features that can be concatenated to the original input:
\begin{align}
    [\B_0 \odot \X, \cdots , \B_k \odot \X, \cdots, \B_{K-1} \odot \X]\in\mathbb{R}^{T \times K}, 
    \label{eq:dct_cat}
\end{align}
where $\mathbf{B} = [\B_0, \cdots, \B_k, \cdots, \B_{K-1}] \in \R^{K \times T}$ is a collection of basis sequences, $K$ is a hyperparameter controlling the complexity of $\mathbf{B}$, and $\odot$ represents the Hadamard (element-wise) product. A larger $k$ corresponds to a basis sequence $\B_k$ with higher frequency. Thus, selecting $K$ close to $T$ leads to \tmodel{} preserving more high-frequency information of $\X$, and vice versa.
To reduce noise, we set $K$ to be small to discard the high-frequency signals from the sequence. As a result, \tmodel{} can capture smooth trajectories of human motions. During implementation, \tmodel{} is applied to each joint's 3D coordinates separately and then concatenated with the existing features. The shape of tensor for an action sequence is changed from $\R^{C \times T \times N \times M}$ to $\R^{(K+1)C \times T \times N \times M}$. As illustrated in \autoref{fig:concept}, \tmodel~can substantially improve the classification accuracy. 
%over concatenating with the other representations. 

In this work, we use the basis of DCT-2. 
% because DCT-2 is exactly equivalent to a DFT up to an overall scaling factor, and DFTs can approximate any temporal trajectory if the basis has sufficient complexity~\cite{}. 
However, a number of other bases, such as those of the discrete Fourier transform or the discrete wavelet transform, can also serve as candidates.
% (wavelet transforms might be particularly applicable to observer-labelled datasets, especially in the spatial domain, due to their more faithful correspondence to human visual processing~\cite{Gaudart:93}).
% Eq (\ref{})
Here, we provide an illustration of why \tmodel{} can increase the flexibility of a neural model. DCTs compute the dot product between sequence $\X$ and basis sequence collection $\mathbf{B}$, as a Hadamard product and a summation, expressed as: 
\begin{align}
    \D_k = \mathbf{1}^\top (\B_k \odot \X), 
\end{align}
where $\mathbf{1} \in \mathbb{R}^K$ is a vector of ones. To facilitate more flexible learning of the frequency information, we replace the summation with a neural network, written as: 
\begin{align}
    \mathbf{d}_\phi = f_\phi(\B_k \odot \X), 
    \label{eq:d_phi}
\end{align}
where $f_\phi$ is a neural network parameterized by $\phi$. Consequently, $\mathbf{d}_\phi$ can extract frequency-related information on an arbitrary subsequence of $\X$ via temporal convolution. For example, convolution over $\B_k \odot \X$ with a $1 \times 3$ filter can learn how much the signals from three consecutive frames align with a given frequency $k$. If we stack multiple temporal convolution layers, the model can then extrapolate frequency information of longer subsequences. 
Note that temporal convolutional layers are commonly employed in skeleton action recognition models~\cite{ji_2013_tpami,li2017skeleton, liu2020disentangling}.
Thus \tmodel{} may improve the performance of most existing models. 
